Depth Field Networks for Generalizable Multi-view Scene Representation

Modern 3D computer vision leverages learning to boost geometric reasoning, mapping image data to classical structures such as cost volumes or epipolar constraints to improve matching. These architectures are specialized according to the particular problem, and thus require significant task-specific tuning, often leading to poor domain generalization performance. Recently, generalist Transformer architectures have achieved impressive results in tasks such as optical flow and depth estimation by encoding geometric priors as inputs rather than as enforced constraints. In this paper, we extend this idea and propose to learn an implicit, multi-view consistent scene representation, introducing a series of 3D data augmentation techniques as a geometric inductive prior to increase view diversity. We also show that introducing view synthesis as an auxiliary task further improves depth estimation. Our Depth Field Networks (DeFiNe) achieve state-of-the-art results in stereo and video depth estimation without explicit geometric constraints, and improve on zero-shot domain generalization by a wide margin.

==> figures/architecture_features.tex <==




\begin{figure}[t!]
\vspace{-3mm}
\renewcommand{\arraystretch}{0.95}
\centering
\subfloat[Depth architecture features.]{
\label{fig:stereo_results}
\raisebox{13mm}{
    \begin{tabular}{l|cccccc}
        \toprule
        Method &
        CV & 
        EP &
        BA &
        OF &
        SN &
        Realtime
 \\
        \toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & & & & & & \textcolor{red}{\xmark}\\
BA-Net (5-view) [2019]~\cite{tang2018ba} & & & \checkmark & & & \textcolor{red}{\xmark} \\
Neural-RGBD [2019]~\cite{liu2019neural} & \checkmark & & & \\ 
DeepV2D [2020]~\cite{deepv2d} & \checkmark & & \checkmark &  \\  
DELTAS [2020]~\cite{sinha2020depth} & & & &  \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  & & \checkmark & &  \\
DRN (refined) [2021]~\cite{ke2021deep} & & & \checkmark & \checkmark \\
MVDepth [2018]~\cite{???} & & & &  \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & &   \\
NAS [2020]~\cite{nas} & & & & \\
EST [2021]~\cite{long2021multi} & \checkmark &  & &  \\
DRN [2021]~\cite{ke2021deep} & &  & & \checkmark &  \\
        \bottomrule
GSR & & & & & & \textcolor{green}{\checkmark}
    \end{tabular}
}
\label{tab:depth_scannet_stereo}
}

\caption{Baseline methods are specialized to depth estimation and use traditional architectures elements.  The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
}
\label{fig:arch_features}
\end{figure}




==> figures/ddad_results.tex <==


\begin{figure}[t!]
\centering
\subfloat{
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_gt_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_gt_rgb.png}
} \\ \vspace{-4mm}
\subfloat{
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_rgb.png}
} \\ \vspace{-4mm}
\subfloat{
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_depth.png}
    \includegraphics[width=0.15\textwidth]{figures/files/ddad_depth.png}
}
\caption{DDAD view and depthh synthesis results. Top: ground-truth images. Middle: predicted RGB values. Bottom: Predicted depth maps.}
\end{figure}

==> figures/encodings.tex <==


% \begin{figure}[t!]
% \centering
% \subfloat[Image Embeddings]{
% \label{fig:rgb_embeddings}
% \includegraphics[width=0.4\textwidth]{figures/files/image_embeddings.png}
% }
% \subfloat[Camera Embeddings]{
% \label{fig:cam_embeddings}
% \includegraphics[width=0.5\textwidth]{figures/files/camera_embeddings.png}
% }
% \caption{
% Embeddings used to encode and decode information. Image embeddings are used \emph{only} at the encoding stage, jointly with camera embeddings. During the decoding stage, only camera embeddings are used to produce synthesized depth and images from novel viewpoints.
% }
% \label{fig:encodings}
% \end{figure}

==> figures/extrapolation.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb0.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb1.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb2.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb3.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb4.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb5.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb6.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb7.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/rgb8.png}}
\vspace{-3mm} \\ 
\subfloat[$t$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel0.png}}
\hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel1.png}}
\hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel2.png}}
\hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel3.png}}
\hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel4.png}}
\hspace{0.1mm}
\subfloat[$t+5$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel5.png}}
\hspace{0.1mm}
\subfloat[$t+6$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel6.png}}
\hspace{0.1mm}
\subfloat[$t+7$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel7.png}}
\hspace{0.1mm}
\subfloat[$t+8$]{\includegraphics[width=0.1\textwidth]{figures/files/extrapolation/novel8.png}}
\caption{Depth extrapolation.}
\end{figure}

==> figures/forecast_all_backup.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
\rotatebox{90}{\hspace{1.0mm} \tiny{RGB}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(0)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(1)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(2)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(3)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(4)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(5)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(6)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(7)_gt.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_rgb(8)_gt.png}} 
\\ 
\rotatebox{90}{\hspace{1.0mm} \tiny{GT}} \!
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(0)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(1)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(2)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(3)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(4)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(5)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(6)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(7)_gt_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(8)_gt_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.4mm} \tiny{Proj.}}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth_valid_gt(8)_pred_viz.png}} 
\\ 
\rotatebox{90}{\hspace{0.1mm} \tiny{Pred.}} \!
\subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(0)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(1)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(2)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(3)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(4)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(5)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(6)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(7)_pred_viz.png}} \hspace{0.1mm}
\subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/26/0000000026_depth(8)_pred_viz.png}}
% \caption{Depth extrapolation.}
% \end{figure}
% \vspace{-2mm} 
% \\
% % \begin{figure}[t!]
% % \captionsetup[subfloat]{labelformat=empty}
% \rotatebox{90}{\hspace{1.5mm} \tiny{RGB}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(0)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(1)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(2)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(3)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(4)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(5)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(6)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(7)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_rgb(8)_gt.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Depth GT}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(0)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(1)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(2)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(3)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(4)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(5)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(6)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(7)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(8)_gt_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Projection}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth_valid_gt(8)_pred_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Predicted}} \!
% \subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3033/0000003033_depth(8)_pred_viz.png}}
% % \caption{Depth extrapolation.}
% % \end{figure}
% \vspace{-2mm} \\
% % \begin{figure}[t!]
% % \captionsetup[subfloat]{labelformat=empty}
% \rotatebox{90}{\hspace{1.5mm} \tiny{RGB}} \!
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(0)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(1)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(2)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(3)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(4)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(5)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(6)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(7)_gt.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_rgb(8)_gt.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Depth GT}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(0)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(1)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(2)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(3)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(4)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(5)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(6)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(7)_gt_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(8)_gt_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Projection}}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth_valid_gt(8)_pred_viz.png}} \vspace{-3mm} \\ 
% \rotatebox{90}{\hspace{0.02mm} \tiny{Predicted}} \!
% \subfloat[$t$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(0)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+1$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(1)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+2$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(2)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+3$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(3)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+4$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(4)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+5$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(5)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+6$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(6)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+7$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(7)_pred_viz.png}} \hspace{0.1mm}
% \subfloat[$t+8$]{\includegraphics[width=0.1\textwidth,height=0.85cm]{figures/files/forecast/3865/0000003865_depth(8)_pred_viz.png}}
\caption{\textbf{ScanNet depth extrapolation examples}, using our proposed GSR architecture. In each example, information from frames at $[t-8,\dots,t-1]$ is encoded, and depth maps corresponding to camera locations at $[t,\dots,t+8]$ are decoded. RGB images and ground-truth depth maps are displayed only for comparison, and not used in these experiments. For each timestep, we show projected ground-truth depth maps (third row), and predicted depth maps (fourth row). Our GSR architecture is able to correctly extrapolate from encoded information to fill in missing parts of the scene.}
\end{figure}

==> figures/interpolation.tex <==

\begin{figure}[t!]
\captionsetup[subfloat]{labelformat=empty}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\vspace{-5mm} \\ 
\subfloat[$t-4$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t-3$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t-2$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t-1$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+1$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+2$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+3$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\hspace{0.1mm}
\subfloat[$t+4$]{\includegraphics[width=0.1\textwidth]{figures/files/virtual/rgb.png}}
\caption{Depth interpolation.}
\label{fig:depth_synthesis}
\end{figure}

==> figures/scannet_stereo_lowres.tex <==



\begin{figure}[t!]
\vspace{-3mm}
\renewcommand{\arraystretch}{0.95}
\centering
\subfloat[Depth estimation results.]{
\label{fig:stereo_results}
\raisebox{13mm}{
    \begin{tabular}{l|cccc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        \small{Sq.Rel}$\downarrow$ &
        RMSE$\downarrow$ &
        $\delta_{1.25}$$\uparrow$
 \\
        \toprule
        DPSNet~\cite{dpsnet} & 0.126 & --- & 0.314 & ---  \\
        NAS~\cite{nas} & 0.107 & --- & 0.281 & ---  \\
        IIB~\cite{yifan2021input} & 0.116 & --- & 0.281 & 0.908  \\
        \midrule
        \textbf{\MethodAcronym} & \textbf{0.089} & \textbf{0.037} & \textbf{0.232} & \textbf{0.915} \\
        \bottomrule
    \end{tabular}
}
\label{tab:depth_scannet_stereo}
}
\hspace{1mm}
\subfloat[Virtual depth estimation results.]{
\label{fig:virtual_results}
    \includegraphics[width=0.4\textwidth, height=2.6cm]{figures/files/virtual_error2.png}
    \label{fig:virtual_error}
}
\caption{\textbf{Depth estimation results on ScanNet-Stereo}. As shown in (a), we outperform other methods by a large margin. In (b) we report depth estimation results on virtual cameras, using different values of $\sigma_v$ at training and test time. 
}
\label{fig:depth_scannet_stereo}
\end{figure}





% \begin{figure}[t!]
% \small
% \centering
% \hspace{5mm}
% \subfloat[View synthesis results]{
%     \begin{tabular}{l|ccc}
%         \toprule
%         \textbf{Method} &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ &
%         LPIPS$\downarrow$ \\
%         \toprule
%         \midrule
%         \textbf{Ours (T)} & 0.714 & 23.810 & - \\
%         \textbf{Ours (C)} & 0.684 & 22.919 & - \\
%         \bottomrule
%     \end{tabular}
% }
% \\
% \subfloat[Depth degradation when rendering depth from different viewpoints.]{
%     \includegraphics[width=0.4\linewidth]{figures/files/virtual_error.png}
% }
% \hspace{5mm}

% % \subfloat[Depth synthesis results]{
% %     \begin{tabular}{l|ccc}
% %         \toprule
% %         \textbf{Method} &
% %         Abs.Rel$\downarrow$ &
% %         RMSE$\downarrow$ &
% %         $\delta_{1.25}$$\uparrow$ \\
% %         \toprule
% %         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- \\
% %         NAS~\cite{nas} & 0.1070 & 0.2807 & --- \\
% %         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 \\
% %         \midrule
% %         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 \\
% %         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 \\
% %         \bottomrule
% %     \end{tabular}
% % }

% \subfloat[Depth synthesis results]{
%     \begin{tabular}{l|ccccc}
%         \toprule
%         \textbf{Method} &
%         Abs.Rel$\downarrow$ &
%         RMSE$\downarrow$ &
%         $\delta_{1.25}$$\uparrow$ &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ \\
%         \toprule
%         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- & &  \\
%         NAS~\cite{nas} & 0.1070 & 0.2807 & --- & &  \\
%         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 & &  \\
%         \midrule
%         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 & & \\
%         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 & &  \\
%         \bottomrule
%     \end{tabular}
% }

% \caption{ScanNet-Stereo results, for depth and view synthesis.}
% \end{figure}

==> figures/scannet_stereo_psnr.tex <==



\begin{figure}[t!]
\renewcommand{\arraystretch}{0.95}
\centering
\subfloat[Depth estimation and view synthesis results.]{
\label{fig:stereo_results}
\raisebox{13mm}{
    \begin{tabular}{l|ccc|cc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        RMSE$\downarrow$ &
        $\delta_{1.25}$$\uparrow$ &
        SSIM$\uparrow$ &
        PSNR$\uparrow$ \\
        \toprule
        DPSNet~\cite{dpsnet} & 0.126 & 0.314 & --- & --- & ---  \\
        NAS~\cite{nas} & 0.107 & 0.281 & --- & --- & ---  \\
        IIB~\cite{yifan2021input} & 0.116 & 0.281 & 0.908 & --- & ---  \\
        \midrule
        \textbf{GSR} & \textbf{0.093} & \textbf{0.246} & \textbf{0.911} & \textbf{0.828} & \textbf{27.727} \\
        \bottomrule
    \end{tabular}
}
\label{tab:depth_scannet_stereo}
}
\hspace{1mm}
\subfloat[Virtual depth estimation results.]{
\label{fig:virtual_results}
    \includegraphics[width=0.36\textwidth, height=3cm]{figures/files/virtual_error.png}
    \label{fig:virtual_error}
}
\caption{\textbf{Depth estimation results on ScanNet-Stereo}. As shown in (a), we outperform other methods by a large margin. In (b) we report depth estimation results on virtual cameras, using different values of $\sigma_v$ at training and test time. 
}
\label{fig:depth_scannet_stereo}
\end{figure}





% \begin{figure}[t!]
% \small
% \centering
% \hspace{5mm}
% \subfloat[View synthesis results]{
%     \begin{tabular}{l|ccc}
%         \toprule
%         \textbf{Method} &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ &
%         LPIPS$\downarrow$ \\
%         \toprule
%         \midrule
%         \textbf{Ours (T)} & 0.714 & 23.810 & - \\
%         \textbf{Ours (C)} & 0.684 & 22.919 & - \\
%         \bottomrule
%     \end{tabular}
% }
% \\
% \subfloat[Depth degradation when rendering depth from different viewpoints.]{
%     \includegraphics[width=0.4\linewidth]{figures/files/virtual_error.png}
% }
% \hspace{5mm}

% % \subfloat[Depth synthesis results]{
% %     \begin{tabular}{l|ccc}
% %         \toprule
% %         \textbf{Method} &
% %         Abs.Rel$\downarrow$ &
% %         RMSE$\downarrow$ &
% %         $\delta_{1.25}$$\uparrow$ \\
% %         \toprule
% %         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- \\
% %         NAS~\cite{nas} & 0.1070 & 0.2807 & --- \\
% %         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 \\
% %         \midrule
% %         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 \\
% %         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 \\
% %         \bottomrule
% %     \end{tabular}
% % }

% \subfloat[Depth synthesis results]{
%     \begin{tabular}{l|ccccc}
%         \toprule
%         \textbf{Method} &
%         Abs.Rel$\downarrow$ &
%         RMSE$\downarrow$ &
%         $\delta_{1.25}$$\uparrow$ &
%         SSIM$\uparrow$ &
%         PSNR$\uparrow$ \\
%         \toprule
%         DPSNet~\cite{dpsnet} & 0.1258 & 0.3145 & --- & &  \\
%         NAS~\cite{nas} & 0.1070 & 0.2807 & --- & &  \\
%         IIB~\cite{yifan2021input} & 0.1159 & 0.2807 & 0.9079 & &  \\
%         \midrule
%         \textbf{Ours (T)} & 0.0982 & 0.2561 & 0.9048 & & \\
%         \textbf{Ours (C)} & 0.1031 & 0.2707 & 0.9016 & &  \\
%         \bottomrule
%     \end{tabular}
% }

% \caption{ScanNet-Stereo results, for depth and view synthesis.}
% \end{figure}

==> figures/scannet_synthesis.tex <==


% \begin{figure}[t!]
% \centering
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/scannet_pcl.png}
% }
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% } \\
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% } \\
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% }
% \caption{DDAD view and depthh synthesis results. Top: ground-truth images. Middle: predicted RGB values. Bottom: Predicted depth maps.}
% \end{figure}

% \begin{figure}[t!]
% \begin{tabular}{cc}
% % \vspace{-30mm}
% % \subfloat{
% % \raisebox{20mm}{\multirow{2}{*}{
% % \vspace{0mm}
% \vspace{10mm}
% \multirow{3}{*}{
% % \raisebox{20mm}{\multirow{2}{*}{
% \includegraphics[width=0.3\columnwidth,height=3cm]{figures/files/scannet_pcl.png}
% % }
% }
% % \\
% % % }
% % % \vspace{-3mm}
% % % \vspace{-30mm}
% % % \\
% % % % \vspace{-30mm}
% % \subfloat[qwer]{
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % }
% % }
% % }
% % }
% & 
% % \raisebox{20mm}{
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% &
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% &
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% % }
% \end{tabular}
% \caption{}
% \end{figure}


% \begin{figure}[t!]
% % \vspace{-30mm}
% % \raisebox{20mm}{\multirow{2}{*}{
% % \subfloat{
% % \raisebox{20mm}{\multirow{2}{*}{
% \subfloat{
% \includegraphics[width=0.3\columnwidth]{figures/files/scannet_pcl.png}
% }
% % }
% % \vspace{-3mm}
% % \vspace{-30mm}
% % \\
% % % \vspace{-30mm}
% % \subfloat[qwer]{
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % \includegraphics[width=0.15\columnwidth]{figures/files/ddad_gt_rgb.png}
% % }
% % }
% % }
% % }
% \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% \\
% % &
% % \subfloat{
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
%     \hspace{1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
%     \hspace{-1mm}
%     \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
% % }
% }
% % \end{tabular}
% \caption{}
% \end{figure}



\begin{figure}[t!]
\begin{tabular}{cc}
% \vspace{10mm}
\raisebox{7mm}{\multirow{3}{*}{
\includegraphics[width=0.3\columnwidth,height=3cm]{figures/files/scannet_pcl.png}
}}
& 
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
\\
&
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
\\
&
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
    \hspace{1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_rgb.png}
    \hspace{-1mm}
    \includegraphics[width=0.1\textwidth]{figures/files/ddad_depth.png}
\end{tabular}
\caption{Depth and view synthesis results on the ScanNet-Stereo dataset.}
\end{figure}

==> figures/scannet_temporal.tex <==



% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|c|c|c|c|c|ccc|c}
        \toprule
        \textbf{Method} &
        CV & EP & BA & OF & SN &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
        \toprule
\multicolumn{6}{l}{\textbf{With test-time refinement}} \\
\toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & & & & & &
0.2310 & 0.5200 & 0.7610 & 110  \\
BA-Net (5-view) [2019]~\cite{tang2018ba} & & & \checkmark & & &  
%0.091 & 0.058 & 0.223 & \underline{95} \\
- & - & - & \underline{95} \\
Neural-RGBD [2019]~\cite{liu2019neural} & \checkmark & & & & &   
0.1013 & 0.0502 & 0.2500 & 195 \\
%DeepV2D [2020]~\cite{deepv2d} & \checkmark & & \checkmark & & &   
%- & - & - & 690 \\
%\textbf{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
DELTAS [2020]~\cite{sinha2020depth} & & & & & &   
0.0915 & 0.0327 & 0.2390 & \textbf{90} \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  & & \checkmark & & & &   
%0.073 & 0.037 & 0.217 & 2400 \\
- & - & - & 2400 \\
DRN (refined) [2021]~\cite{ke2021deep} & & & \checkmark & \checkmark & &   
- & - & - & 168 \\
%\underline{0.058} & \underline{0.018} & \textbf{0.162} & 168 \\
\midrule
\multicolumn{6}{l}{\textbf{Without test-time refinement}} \\
\midrule
MVDepth [2018]~\cite{???} & & & & & &   
0.1167 & 0.0596 & 0.3236 & - \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & & & &   
0.2080 & 0.3180 & 0.7420 & - \\
NAS [2020]~\cite{nas} & & & & & &   
0.0941 & 0.0417 & 0.2703 & - \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
EST [2021]~\cite{long2021multi} & \checkmark &  & & & &   
0.0812 & 0.0298 & 0.2199 & 71 \\
%\midrule
DRN [2021]~\cite{ke2021deep} & &  & & \checkmark & &   
%\underline{0.068} & \underline{0.026} & \textbf{0.178} & - \\
- & - & - & - \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
% | DEPTH|GT(0_0)_0                |  0.063   |  0.024   |  0.194   |  0.093   |  8.987   |  0.952   |  0.990   |  0.998   |  0.910   | 
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}} \\
\midrule
MVDepth [2018]~\cite{???} & \checkmark & & & & &   
0.2213 & 0.2401 & 0.5154 & - \\
DPSNet [2019]~\cite{dpsnet} & \checkmark & & & & &   
0.1963 & 0.1970 & 0.4625 & 225 \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
NAS [2020]~\cite{nas} & & \checkmark & & & \checkmark &   
0.1631 & 0.1023 & 0.3791 & - \\
EST [2021]~\cite{yifan2021input} & \checkmark &  & & & &   
0.1465 & 0.0729 & 0.3382 & 71 \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet}. We separate methods that include test-time refinement (e.g. windowed bundle adjustment) from those that, similar to ours, do not refine at test time. We also include zero-shot transfer results to 7~Scenes. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
%Results trained on the full Scannet dataset, trained and evaluated with window size of [-X,X].  The $\dagger$ indicates test-time optimization, while GRS is only a forward pass.
}
\vspace{-3mm}
\label{fig:depth_scannet_temporal}
\end{table}


        %  & 0.196 & 0.197 & 0.463  \\
        %  & 0.163 & 0.102 & 0.379   \\
        %  & 0.147 & 0.073 & 0.338   \\
        % \midrule
        % \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\



==> figures/scannet_temporal_deepv2d_align.tex <==
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|ccc|c}
        \toprule
        \textbf{Method} &
        \small{Abs.\ Rel}$\downarrow$ &
        Sq.\ Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{ScanNet test split} \cite{tang2018ba}} \\
\midrule
DeMoN [2017]~\cite{ummenhofer2017demon} &
0.231 & 0.520 & 0.761 & 110  \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & 
0.208 & 0.318 & 0.742 & - \\
BA-Net [2019]~\cite{tang2018ba} &
0.091 & 0.058 & 0.223 & 95 \\
CVD [2020]~\cite{luo2020consistent} &   
0.073 & 0.037 & 0.217 & 2400 \\
DeepV2D [2020]~\cite{deepv2d} &  
\underline{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} & 
\textbf{0.047} & 0.024 & \textbf{0.164} & \textbf{30} \\
\midrule
\textbf{\MethodAcronym} ($128 \times 192$)&
0.059 & 0.022 & 0.184 &  \underline{49} \\
\textbf{\MethodAcronym} ($240 \times 320$) &
\underline{0.057} & \underline{0.019} & 0.178 &  78 \\

\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}~\cite{shotton2013scene}} \\
\midrule
DeMoN [2017]~\cite{ummenhofer2017demon} &  
0.389 & 0.420 & 0.855 & 110 \\
NeuralRGBD [2019]~\cite{liu2019neural} &
0.176 & 0.112 & 0.441 & 202 \\
DPSNet [2019]~\cite{dpsnet} &  
0.199 & 0.142 & 0.438  & 322 \\
DeepV2D [2020]~\cite{deepv2d} &  
0.437 & 0.553 & 0.869  & 347 \\
CNMNet [2020]~\cite{long2020occlusion} &   
0.161 & 0.083 & 0.361 & 80 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} &  
0.155 & 0.104 & 0.347 & \textbf{30} \\
EST [2021]~\cite{yifan2021input} &  
\underline{0.118} & \underline{0.052} & \underline{0.298} & 71 \\
\midrule
\textbf{\MethodAcronym} & 
\textbf{0.100} & \textbf{0.039} & \textbf{0.253} &  \underline{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet and 7~Scenes}. 
\MethodAcronym is competitive with other state-of-the-art methods on ScanNet, and outperforms all published methods in zero-shot transfer to 7~Scenes by a large margin.
}
\vspace{-10mm}
\label{tab:depth_scannet_temporal}
\end{table}



==> figures/scannet_temporal_deev2d_checkmarks.tex <==

% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|cccc|ccc|c}
        \toprule
        \textbf{Method} &
        CV & EP & BA & SN &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{ScanNet test split} \cite{tang2018ba}} \\
\midrule
DeMoN$^\dagger$ [2017]~\cite{ummenhofer2017demon} & & & & & 
0.231 & 0.520 & 0.761 & 110  \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & & &  
0.208 & 0.318 & 0.742 & - \\
BA-Net$^\dagger$ (5-view) [2019]~\cite{tang2018ba} & & & \textcolor{red}{\checkmark} & & 
0.091 & 0.058 & 0.223 & 95 \\
CVD$^\dagger$ [2020]~\cite{luo2020consistent} & & \textcolor{red}{\checkmark} & & &   
0.073 & 0.037 & 0.217 & 2400 \\
DeepV2D$^\dagger$ [2020]~\cite{deepv2d} & \textcolor{red}{\checkmark}  & & \textcolor{red}{\checkmark} & &   
\underline{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} & & & & \textcolor{red}{\checkmark} &  
\textbf{0.047} & 0.024 & \textbf{0.164} & \textbf{30} \\
\midrule
\textbf{GSR} & & & & & 
0.059 & \underline{0.020} & 0.183 &  \underline{49} \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}~\cite{shotton2013scene}} \\
\midrule
DeMoN [2017]~\cite{ummenhofer2017demon} &  & & & & 
0.389 & 0.420 & 0.855 & 110 \\
% MVSNet [2018]~\cite{yao2018mvsnet} &   
% 0.234 & 0.190 & 0.508 & 1050 \\
NeuralRGBD [2019]~\cite{liu2019neural} & \textcolor{red}{\checkmark}  & & & & 
0.176 & 0.112 & 0.441 & 202 \\
% MVDNet [2018]~\cite{wang2018mvdepthnet} &  
% 0.193 & 0.235 & 0.459 & \underline{48} \\
DPSNet [2019]~\cite{dpsnet} & \textcolor{red}{\checkmark}  & & & & 
0.199 & 0.142 & 0.438  & 322 \\
DeepV2D [2020]~\cite{deepv2d} & \textcolor{red}{\checkmark}  & & \textcolor{red}{\checkmark} & &  
0.437 & 0.553 & 0.869  & 347 \\
CNMNet [2020]~\cite{long2020occlusion} & \textcolor{red}{\checkmark} & & & &    
0.161 & 0.083 & 0.361 & 80 \\
NeuralRecon [2021]~\cite{Sun_2021_CVPR} & & & & \textcolor{red}{\checkmark} &   
0.155 & 0.104 & 0.347 & \textbf{30} \\
EST [2021]~\cite{yifan2021input} & \textcolor{red}{\checkmark} & & & &    
\underline{0.118} & \underline{0.052} & \underline{0.298} & 71 \\
\midrule
\textbf{GSR} & & & & & 
\textbf{0.100} & \textbf{0.039} & \textbf{0.253} &  \underline{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet and 7~Scenes}. 
The symbol $^\dagger$ indicates the use of test-time optimization. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), and SDF volumes (SV).
}
\vspace{-10mm}
\label{fig:depth_scannet_temporal}
\end{table}



==> figures/scannet_temporal_scaled.tex <==



% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|ccc|c}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
        \toprule
\multicolumn{6}{l}{\textbf{With test-time refinement}} \\
\toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & 
0.231 & 0.520 & 0.761 & 110  \\
BA-Net (5-view) [2019]~\cite{tang2018ba} &  
0.091 & 0.058 & 0.223 & \underline{95} \\
Neural-RGBD [2019]~\cite{liu2019neural} &  
0.097 & 0.050 & 0.249 & 195 \\
DeepV2D [2020]~\cite{deepv2d} & 
\textbf{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
DELTAS [2020]~\cite{sinha2020depth} & 
0.092 & 0.033 & 0.234 & \textbf{90} \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  &  
0.073 & 0.037 & 0.217 & 2400 \\
DRN (refined) [2021]~\cite{ke2021deep} &  
\underline{0.058} & \underline{0.018} & \textbf{0.162} & 168 \\
\midrule
\multicolumn{6}{l}{\textbf{Without test-time refinement}} \\
\midrule
MiDas-v2 [2019]~\cite{ranftl2020towards} & 
0.208 & 0.318 & 0.742 & - \\
EST [2021]~\cite{long2021multi} &  
0.081 & 0.030 & 0.220 & 71 \\
%\midrule
DRN [2021]~\cite{ke2021deep} &  
\underline{0.068} & \underline{0.026} & \textbf{0.178} & - \\
\textbf{GSR} & & & & & &  
\textbf{0.063} & \textbf{0.024} & \underline{0.194} &  \textbf{49} \\
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}} \\
\midrule
DPSNet [2019]~\cite{dpsnet} & 
0.196 & 0.197 & 0.463 & 225 \\
NAS [2020]~\cite{nas} & 
0.163 & 0.102 & 0.379 & - \\
EST [2021]~\cite{yifan2021input} &  
\underline{0.147} & \underline{0.073} & \underline{0.338} & 71 \\
\textbf{GSR} & 
\textbf{0.106} & \textbf{0.044} & \textbf{0.267} &  \textbf{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet}. We separate methods that include test-time refinement (e.g. windowed bundle adjustment) from those that, similar to ours, do not refine at test time. We also include zero-shot transfer results to 7~Scenes. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
%Results trained on the full Scannet dataset, trained and evaluated with window size of [-X,X].  The $\dagger$ indicates test-time optimization, while GRS is only a forward pass.
}
\vspace{-3mm}
\label{fig:depth_scannet_temporal}
\end{table}


        %  & 0.196 & 0.197 & 0.463  \\
        %  & 0.163 & 0.102 & 0.379   \\
        %  & 0.147 & 0.073 & 0.338   \\
        % \midrule
        % \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\



==> figures/scannet_temporal_unscaled.tex <==



% \begin{figure}
\begin{table}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
    \begin{tabular}{l|c|c|c|c|c|ccc|c}
        \toprule
        \textbf{Method} &
        CV & EP & BA & OF & SN &
        \small{Abs.Rel}$\downarrow$ &
        Sq Rel$\downarrow$ &
        RMSE$\downarrow$ & Speed (ms)$\downarrow$
        \\
        \toprule
\multicolumn{6}{l}{\textbf{With test-time refinement}} \\
\toprule
DeMoN [2017]~\cite{ummenhofer2017demon} & & & & & &
0.2310 & 0.5200 & 0.7610 & 110  \\
BA-Net (5-view) [2019]~\cite{tang2018ba} & & & \checkmark & & &  
%0.091 & 0.058 & 0.223 & \underline{95} \\
- & - & - & \underline{95} \\
Neural-RGBD [2019]~\cite{liu2019neural} & \checkmark & & & & &   
0.1013 & 0.0502 & 0.2500 & 195 \\
%DeepV2D [2020]~\cite{deepv2d} & \checkmark & & \checkmark & & &   
%- & - & - & 690 \\
%\textbf{0.057} & \textbf{0.010} & \underline{0.168} & 690 \\
DELTAS [2020]~\cite{sinha2020depth} & & & & & &   
0.0915 & 0.0327 & 0.2390 & \textbf{90} \\
CVD [2020]~\cite{luo2020consistent}$\dagger$  & & \checkmark & & & &   
%0.073 & 0.037 & 0.217 & 2400 \\
- & - & - & 2400 \\
DRN (refined) [2021]~\cite{ke2021deep} & & & \checkmark & \checkmark & &   
- & - & - & 168 \\
%\underline{0.058} & \underline{0.018} & \textbf{0.162} & 168 \\
\midrule
\multicolumn{6}{l}{\textbf{Without test-time refinement}} \\
\midrule
MVDepth [2018]~\cite{???} & & & & & &   
0.1167 & 0.0596 & 0.3236 & - \\
MiDas-v2 [2019]~\cite{ranftl2020towards} & & & & & &   
0.2080 & 0.3180 & 0.7420 & - \\
NAS [2020]~\cite{nas} & & & & & &   
0.0941 & 0.0417 & 0.2703 & - \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
EST [2021]~\cite{long2021multi} & \checkmark &  & & & &   
0.0812 & 0.0298 & 0.2199 & 71 \\
%\midrule
DRN [2021]~\cite{ke2021deep} & &  & & \checkmark & &   
%\underline{0.068} & \underline{0.026} & \textbf{0.178} & - \\
- & - & - & - \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
% | DEPTH|GT(0_0)_0                |  0.063   |  0.024   |  0.194   |  0.093   |  8.987   |  0.952   |  0.990   |  0.998   |  0.910   | 
\midrule
\midrule
\multicolumn{6}{l}{\textbf{Zero-shot transfer to 7~Scenes}} \\
\midrule
MVDepth [2018]~\cite{???} & \checkmark & & & & &   
0.2213 & 0.2401 & 0.5154 & - \\
DPSNet [2019]~\cite{dpsnet} & \checkmark & & & & &   
0.1963 & 0.1970 & 0.4625 & 225 \\
%EST [2021]~\cite{long2021multi} & & \checkmark & &   
%0.058 & 0.018 & 0.018 &
NAS [2020]~\cite{nas} & & \checkmark & & & \checkmark &   
0.1631 & 0.1023 & 0.3791 & - \\
EST [2021]~\cite{yifan2021input} & \checkmark &  & & & &   
0.1465 & 0.0729 & 0.3382 & 71 \\
\textbf{GSR} & & & & & &  
- & - & - &  \textbf{49} \\
\bottomrule
\end{tabular}
\caption{\textbf{Depth estimation results on ScanNet}. We separate methods that include test-time refinement (e.g. windowed bundle adjustment) from those that, similar to ours, do not refine at test time. We also include zero-shot transfer results to 7~Scenes. The checkmarks indicate the use of cost volumes (CV), epipolar constraints (EP), bundle-adjustment (BA), optical flow estimation (OF), and surface normal estimation (SN).
%Results trained on the full Scannet dataset, trained and evaluated with window size of [-X,X].  The $\dagger$ indicates test-time optimization, while GRS is only a forward pass.
}
\vspace{-3mm}
\label{fig:depth_scannet_temporal}
\end{table}


        %  & 0.196 & 0.197 & 0.463  \\
        %  & 0.163 & 0.102 & 0.379   \\
        %  & 0.147 & 0.073 & 0.338   \\
        % \midrule
        % \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\



==> figures/seven_scenes.tex <==
\begin{figure}[t!]
%\begin{minipage}[c]{.5\textwidth}
\centering
\label{fig:sevenscenes_results}
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        Sq. Rel$\downarrow$ &
        RMSE$\downarrow$ \\
        \toprule
        DPSNet~\cite{dpsnet} & 0.196 & 0.197 & 0.463  \\
        NAS~\cite{nas} & 0.163 & 0.102 & 0.379   \\
        EST~\cite{yifan2021input} & 0.147 & 0.073 & 0.338   \\
        \midrule
        \textbf{GSR} & \textbf{0.106} & \textbf{0.044} & \textbf{0.267}  \\
        \bottomrule
    \end{tabular}
%\end{minipage}%
%\begin{minipage}[c]{.5\textwidth}
\caption{\textbf{Depth estimation results on 7~Scenes}.  Models trained on the Scannet train set and tested on the 7~Scenes test set sequences.}
%}
\label{fig:depth_scannet_stereo}
%\end{minipage}
\end{figure}



==> figures/virtual.tex <==

\begin{figure}[t!]
\begin{tabular}{cc}
% \vspace{10mm}
\raisebox{9mm}{\multirow{2}{*}{
\includegraphics[width=0.3\columnwidth,height=2.5cm]{figures/files/scannet_pcl.png}
}}
& 
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/rgb.png}
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/rgb1.png}
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/rgb2.png}
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/rgb3.png}
\\
&
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/depth.png}
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/depth1.png}
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/depth2.png}
    \includegraphics[width=0.15\textwidth]{figures/files/virtual/depth3.png}
\end{tabular}
\caption{Examples of virtual camera augmentations.}
\end{figure}

==> tables/ablation_psnr.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{0.92}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccc|cc}
\toprule
\multirow{2}{*}{\textbf{Variation}} &
\multicolumn{4}{c}{Depth} &
\multicolumn{2}{c}{View} \\
& 
Abs.Rel &
Sqr.Rel &
RMSE &
$\delta_{1.25}$ &
SSIM & 
PSNR \\
\toprule
Depth-Only & 0.098 & 0.046 & 0.257 & 0.902 & -- & -- \\
RGB-Only & -- & -- & -- & -- & 0.576 & 21.071 \\
\midrule
w/ Conv. RGB encoder & 0.114 & 0.058 & 0.294 & 0.866 & 0.644 & 23.151 \\
w/ 64-dim R18 RGB encoder & 0.104 & 0.049 & 0.270 & 0.883 & 0.675 & 23.859 \\
\midrule
w/o camera information & 0.229 & 0.157 & 0.473 & 0.661 & 0.606 & 16.924 \\
w/o global rays encoding & 0.097 & 0.047 & 0.261 & 0.897 & 0.788 & 26.267 \\
w/ equal loss weights & 0.095 & 0.047 & 0.259 & 0.908 & 0.736 & 24.621 \\
w/ epipolar cues~\cite{yifan2021input} & 0.094 & 0.048 & 0.254 & 0.905 & 0.798 & 26.998 \\
\midrule
w/o Augmentations & 0.117 & 0.060 & 0.291 & 0.870 & 0.741 & 24.758 \\
w/o Virtual Cameras & 0.104 & 0.058 & 0.268 & 0.891 & 0.770 & 25.274 \\
w/o Canonical Jittering & 0.099 & 0.046 & 0.261 & 0.897 & 0.788 & 26.267 \\
w/o Canonical Randomization & 0.096 & 0.044 & 0.253 & 0.905 & 0.792 & 26.284 \\
\midrule
% Ours ($T_1$) & 0.097 & 0.258 & 0.905 & 0.816 & 27.120  \\
\textbf{GSR} & \textbf{0.093} & \textbf{0.042} & \textbf{0.246} & \textbf{0.911} & \textbf{0.828} & \textbf{27.727} \\
\bottomrule
\end{tabular}
}
\caption{Ablation table for ScanNet-Stereo, using different GSR variations. } 
\label{tab:ablation}
\vspace{-5mm}
\end{table*}



==> tables/depth_multi_camera.tex <==


\begin{table*}[t!]
\small
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|ccccc|ccc}
\toprule
& \multirow{2}{*}{\textbf{Camera}} &
\multicolumn{5}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& &
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textit{Method}}}} 
& 01 & & & & & & & & \\
& 05 & & & & & & & & \\
& 06 & & & & & & & & \\
& 07 & & & & & & & & \\
& 08 & & & & & & & & \\
& 09 & & & & & & & & \\
\bottomrule
\end{tabular}
}
\caption{Placeholder multi-camera depth table.} 
\label{tab:depth_multi_camera}
\end{table*}




==> tables/depth_single_camera.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{5}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& 
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
SILog & 
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule
& & & & & & & & 
\\

\bottomrule

\end{tabular}
}
\caption{Placeholder single camera depth table.} 
\label{tab:depth_single_camera}
\end{table*}



==> tables/extrapolation.tex <==



\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccccccc}
% \toprule
% Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
% \midrule
% \% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
% \toprule
% Monodepth2 & 0.164 & 0.178 & 0.188 & 0.194 & 0.201 & 0.208 & 0.215 & 0.221 & 0.228 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GRS (projection) & 0.132 & 0.147 & 0.154 & 0.162 & 0.168 & 0.177 & 0.184 & 0.191 & 0.198 \\
% GRS (novel) & 0.131 & 0.144 & 0.151 & 0.158 & 0.165 & 0.172 & 0.178 & 0.184 & 0.190 \\
% \midrule
% \midrule
% GRS (novel, all) & 0.138 & 0.159 & 0.175 & 0.192 & 0.209 & 0.224 & 0.238 & 0.251 & 0.263 \\
% \bottomrule
\toprule
Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
\midrule
\% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
\toprule
Monodepth2 & 0.351 & 0.386 & 0.398 & 0.405 & 0.412 & 0.420 & 0.431 & 0.441 & 0.453 \\
PackNet & 0.327 & 0.358 & 0.378 & 0.391 & 0.400 & 0.406 & 0.420 & 0.428 & 0.436 \\
BTS & 0.315 & 0.331 & 0.357 & 0.377 & 0.392 & 0.401 & 0.413 & 0.424 & 0.429 \\
\midrule
DeFiNe (projection) & 0.258 & 0.276 & 0.288 & 0.298 & 0.311 & 0.323 & 0.331 & 0.340 & 0.348 \\
DeFiNe (query) & 0.237 & 0.260 & 0.271 & 0.280 & 0.289 & 0.298 & 0.307 & 0.317 & 0.326 \\
\midrule
\midrule
DeFiNe (query, all) & 0.326 & 0.370 & 0.405 & 0.438 & 0.468 & 0.495 & 0.520 & 0.543 & 0.563 \\
\bottomrule
\end{tabular}
}
\caption{Depth extrapolation (Abs.\ Rel).} 
\label{tab:extrapolation}
\end{table*}


% \begin{table*}[t!]
% %\vspace{-4mm}
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|ccccccccc}
% \toprule
% Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
% \midrule
% \% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
% \toprule
% Monodepth2 & 0.421 & 0.456 & 0.468 & 0.475 & 0.482 & 0.490 & 0.501 & 0.511 & 0.521 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GRS (projection) & - & - & - & - & - & - & - & - & - \\
% GRS (novel) & - & - & - & - & - & - & - & - & - \\
% \midrule
% \midrule
% GRS (novel, all) & - & - & - & - & - & - & - & - & - \\
% \bottomrule
% \end{tabular}
% }
% \caption{Depth extrapolation (RMSE).} 
% \label{tab:extrapolation}
% \end{table*}








% \begin{table*}[t!]
% %\vspace{-4mm}
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|ccccccccc}
% % \toprule
% % Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
% % \midrule
% % \% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
% % \toprule
% % Monodepth2 & 0.164 & 0.178 & 0.188 & 0.194 & 0.201 & 0.208 & 0.215 & 0.221 & 0.228 \\
% % PackNet & - & - & - & - & - & - & - & - & - \\
% % BTS & - & - & - & - & - & - & - & - & - \\
% % \midrule
% % GRS (projection) & 0.132 & 0.147 & 0.154 & 0.162 & 0.168 & 0.177 & 0.184 & 0.191 & 0.198 \\
% % GRS (novel) & 0.131 & 0.144 & 0.151 & 0.158 & 0.165 & 0.172 & 0.178 & 0.184 & 0.190 \\
% % \midrule
% % \midrule
% % GRS (novel, all) & 0.138 & 0.159 & 0.175 & 0.192 & 0.209 & 0.224 & 0.238 & 0.251 & 0.263 \\
% % \bottomrule
% \toprule
% Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
% \midrule
% \% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
% \toprule
% Monodepth2 & 0.421 & 0.456 & 0.468 & 0.475 & 0.482 & 0.490 & 0.501 & 0.511 & 0.521 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GRS (projection) & 0.330 & 0.349 & 0.358 & 0.367 & 0.376 & 0.385 & 0.394 & 0.403 & 0.413 \\
% GRS (novel) & 0.312 & 0.333 & 0.343 & 0.350 & 0.362 & 0.372 & 0.382 & 0.388 & 0.396 \\
% \midrule
% \midrule
% GRS (novel, all) & 0.330 & 0.372 & 0.406 & 0.439 & 0.470 & 0.497 & 0.522 & 0.545 & 0.565 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Depth extrapolation (Abs.Rel).} 
% \label{tab:extrapolation}
% \end{table*}


% % \begin{table*}[t!]
% % %\vspace{-4mm}
% % \renewcommand{\arraystretch}{0.9}
% % \centering
% % {
% % \small
% % \setlength{\tabcolsep}{0.3em}
% % \begin{tabular}{l|ccccccccc}
% % \toprule
% % Timestep & $0$ & $1$ & $2$ & $3$ & $4$ & $5$ & $6$ & $7$ & $8$ \\
% % \midrule
% % \% valid pixels & $91.0$ & $76.1$ & $64.5$ & $55.9$ & $49.6$ & $45.2$ & $42.0$ & $39.5$ & $36.0$ \\
% % \toprule
% % Monodepth2 & 0.421 & 0.456 & 0.468 & 0.475 & 0.482 & 0.490 & 0.501 & 0.511 & 0.521 \\
% % PackNet & - & - & - & - & - & - & - & - & - \\
% % BTS & - & - & - & - & - & - & - & - & - \\
% % \midrule
% % GRS (projection) & - & - & - & - & - & - & - & - & - \\
% % GRS (novel) & - & - & - & - & - & - & - & - & - \\
% % \midrule
% % \midrule
% % GRS (novel, all) & - & - & - & - & - & - & - & - & - \\
% % \bottomrule
% % \end{tabular}
% % }
% % \caption{Depth extrapolation (RMSE).} 
% % \label{tab:extrapolation}
% % \end{table*}



==> tables/interpolation.tex <==



\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{0.9}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccccccc}
% \toprule
% Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
% \midrule
% \% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
% \toprule
% Monodepth2 & 0.168 & 0.179 & 0.186 & 0.193 & 0.200 & 0.196 & 0.190 & 0.183 & 0.172 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GRS (projection) & 0.138 & 0.146 & 0.155 & 0.162 & 0.165 & 0.163 & 0.158 & 0.150 & 0.139 \\
% GRS (novel) & 0.138 & 0.148 & 0.154 & 0.158 & 0.161 & 0.157 & 0.154 & 0.148 & 0.137 \\
% \midrule
% \midrule
% GRS (novel, all) & 0.150 & 0.159 & 0.166 & 0.172 & 0.176 & 0.174 & 0.171 & 0.163 & 0.153 \\
% \bottomrule
\toprule
Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
\midrule
\% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
\toprule
Monodepth2 & 0.325 & 0.336 & 0.346 & 0.354 & 0.361 & 0.359 & 0.354 & 0.347 & 0.338 \\
PackNet    & 0.305 & 0.318 & 0.330 & 0.341 & 0.344 & 0.344 & 0.336 & 0.327 & 0.338 \\
BTS        & 0.296 & 0.306 & 0.320 & 0.329 & 0.334 & 0.326 & 0.327 & 0.319 & 0.303 \\
\midrule
DeFiNe (projection) & 0.226 & 0.239 & 0.251 & 0.259 & 0.268 & 0.261 & 0.254 & 0.244 & 0.231 \\
DeFiNe (query)      & 0.222 & 0.230 & 0.237 & 0.240 & 0.242 & 0.246 & 0.245 & 0.240 & 0.231 \\
\midrule
\midrule
DeFiNe (query, all) & 0.361 & 0.381 & 0.398 & 0.408 & 0.412 & 0.413 & 0.406 & 0.390 & 0.369 \\
\bottomrule
\end{tabular}
}
\caption{Depth Interpolation.} 
\label{tab:interpolation}
\end{table*}


% \begin{table*}[t!]
% %\vspace{-4mm}
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|ccccccccc}
% \toprule
% Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
% \midrule
% \% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
% \toprule
% Monodepth2 & 0.436 & 0.455 & 0.466 & 0.476 & 0.484 & 0.477 & 0.468 & 0.448 & 0.433 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GRS (projection) & 0.366 & 0.376 & 0.386 & 0.392 & 0.390 & 0.395 & 0.0.382 & 0.371 & 0.354 \\
% GRS (novel) & 0.347 & 0.351 & 0.362 & 0.375 & 0.382 & 0.379 & 0.366 & 0.358 & 0.349 \\
% \midrule
% \midrule
% GRS (novel, all) & 0.350 & 0.369 & 0.384 & 0.392 & 0.394 & 0.396 & 0.389 & 0.375 & 0.356 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Depth Interpolation (RMSE).} 
% \label{tab:interpolation}
% \end{table*}








% \begin{table*}[t!]
% %\vspace{-4mm}
% \renewcommand{\arraystretch}{0.9}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|ccccccccc}
% % \toprule
% % Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
% % \midrule
% % \% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
% % \toprule
% % Monodepth2 & 0.168 & 0.179 & 0.186 & 0.193 & 0.200 & 0.196 & 0.190 & 0.183 & 0.172 \\
% % PackNet & - & - & - & - & - & - & - & - & - \\
% % BTS & - & - & - & - & - & - & - & - & - \\
% % \midrule
% % GRS (projection) & 0.138 & 0.146 & 0.155 & 0.162 & 0.165 & 0.163 & 0.158 & 0.150 & 0.139 \\
% % GRS (novel) & 0.138 & 0.148 & 0.154 & 0.158 & 0.161 & 0.157 & 0.154 & 0.148 & 0.137 \\
% % \midrule
% % \midrule
% % GRS (novel, all) & 0.150 & 0.159 & 0.166 & 0.172 & 0.176 & 0.174 & 0.171 & 0.163 & 0.153 \\
% % \bottomrule
% \toprule
% Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
% \midrule
% \% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
% \toprule
% Monodepth2 & 0.436 & 0.455 & 0.466 & 0.476 & 0.484 & 0.477 & 0.468 & 0.448 & 0.433 \\
% PackNet & - & - & - & - & - & - & - & - & - \\
% BTS & - & - & - & - & - & - & - & - & - \\
% \midrule
% GSR (projection) & 0.366 & 0.376 & 0.386 & 0.392 & 0.390 & 0.395 & 0.0.382 & 0.371 & 0.354 \\
% GSR (novel) & 0.347 & 0.351 & 0.362 & 0.375 & 0.382 & 0.379 & 0.366 & 0.358 & 0.349 \\
% \midrule
% \midrule
% GSR (novel, all) & 0.350 & 0.369 & 0.384 & 0.392 & 0.394 & 0.396 & 0.389 & 0.375 & 0.356 \\
% \bottomrule
% \end{tabular}
% }
% \caption{Depth Interpolation.} 
% \label{tab:interpolation}
% \end{table*}


% % \begin{table*}[t!]
% % %\vspace{-4mm}
% % \renewcommand{\arraystretch}{0.9}
% % \centering
% % {
% % \small
% % \setlength{\tabcolsep}{0.3em}
% % \begin{tabular}{l|ccccccccc}
% % \toprule
% % Timestep & $-4$ & $-3$ & $-2$ & $-1$ & $0$ & $+1$ & $+2$ & $+3$ & $+4$ \\
% % \midrule
% % \% valid pixels & $77.7$ & $68.5$ & $62.6$ & $59.5$ & $58.2$ & $58.7$ & $61.2$ & $66.6$ & $75.9$ \\
% % \toprule
% % Monodepth2 & 0.436 & 0.455 & 0.466 & 0.476 & 0.484 & 0.477 & 0.468 & 0.448 & 0.433 \\
% % PackNet & - & - & - & - & - & - & - & - & - \\
% % BTS & - & - & - & - & - & - & - & - & - \\
% % \midrule
% % GRS (projection) & 0.366 & 0.376 & 0.386 & 0.392 & 0.390 & 0.395 & 0.0.382 & 0.371 & 0.354 \\
% % GRS (novel) & 0.347 & 0.351 & 0.362 & 0.375 & 0.382 & 0.379 & 0.366 & 0.358 & 0.349 \\
% % \midrule
% % \midrule
% % GRS (novel, all) & 0.350 & 0.369 & 0.384 & 0.392 & 0.394 & 0.396 & 0.389 & 0.375 & 0.356 \\
% % \bottomrule
% % \end{tabular}
% % }
% % \caption{Depth Interpolation (RMSE).} 
% % \label{tab:interpolation}
% % \end{table*}


==> tables/monocular_ablations.tex <==
\begin{figure}[t!]
\centering
\label{fig:monocular_results}
    \begin{tabular}{l|ccc}
        \toprule
        \textbf{Method} &
        \small{Abs.Rel}$\downarrow$ &
        % \small{Sq.Rel}$\downarrow$ &
        RMSE$\downarrow$ &
        $\delta_{1.25}$$\uparrow$ \\
        \toprule
        No Aug. & 0.149 & 0.078 & 0.806  \\
        3D Aug. & X & X & X  \\
        \midrule
        IIB~\cite{yifan2021input} & 0.116  & 0.281 & 0.908  \\
        \textbf{\MethodAcronym} & \textbf{0.089} & \textbf{0.232} & \textbf{0.915} \\
        \bottomrule
    \end{tabular}
\caption{Comparing \textbf{monocular depth} training to IIB and DeFiNe.}
\end{figure}

==> tables/scannet_viewsynth.tex <==

\begin{table*}[t!]
%\vspace{-4mm}
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|ccccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{5}{|c|}{Higher is better $\uparrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& 
PSNR &
LPIPS &
SSIM &
%RMSE$_{log}$ &
%SILog & 
%$\delta<1.25$ &
%$\delta<1.25^2$ &
%$\delta<1.25^3$\vspace{0.5mm}\\
\\
\toprule
PerspectiveNet & 13.986 & 0.426 & & & & & & 
\\

\bottomrule

\end{tabular}
}
\caption{View synthesis results on ScanNet.} 
\label{tab:scannet_view_synthesis}
\end{table*}


